Practical Implementation of Spatial Modulation

In this work we seek to characterise the performance of spatial modulation (SM) and spatial multiplexing (SMX) with an experimental test bed. Two National Instruments (NI)-PXIe devices are used for the system testing, one for the transmitter and one for the receiver. The digital signal processing that formats the information data in preparation of transmission is described along with the digital signal processing that recovers the information data. In addition, the hardware limitations of the system are also analysed. The average bit error ratio (ABER) of the system is validated through both theoretical analysis and simulation results for SM and SMX under line of sight (LoS) channel conditions.

==> Biographies/Abdelhamid_Younis.tex <==
Abdelhamid Younis received a BSc in Electrical and Electronic Engineering with honours in 2007 from the University of Benghazi, Libya and an MSc with distinction in Signal Processing and Communication Engineering in 2009 from the University of Edinburgh, UK. He is currently completing a Ph.D. in Communication Engineering at the Institute of Digital Communications (IDCOM) at the University of Edinburgh where in 2010 he was awarded the Overseas Research Student Award (ORS) in recognition of his work. His main research interests lie in the area of wireless communication and digital signal processing with a particular focus on spatial modulation, MIMO wireless communications, reduced complexity MIMO design and optical wireless communications.


==> Biographies/Cheng_Xiang_Wang.tex <==
Cheng-Xiang~Wang (S'01-M'05-SM'08) received the BSc and MEng degrees in Communication and Information Systems from Shandong University, China, in 1997 and 2000, respectively, and the PhD degree in Wireless Communications
from Aalborg University, Denmark, in 2004.
 
He has been with Heriot-Watt University, Edinburgh, UK, since 2005, first as a Lecturer, then as a Reader in 2009, and was promoted to a Professor in 2011. He is also an Honorary Fellow of the University of Edinburgh, UK, and a Chair/Guest Professor of Shandong University, Huazhong University of Science and Technology, and Southeast University, China. He was a Research Fellow at the University of Agder, Grimstad, Norway, from 2001--2005, a Visiting Researcher at Siemens AG-Mobile Phones, Munich, Germany, in 2004, and a Research Assistant at Technical University of Hamburg-Harburg, Hamburg, Germany, from 2000--2001. His current research interests include wireless channel modeling and simulation, green communications, cognitive radio networks, vehicular communication networks, Large MIMO, cooperative MIMO, and B4G wireless communications. He has published 1 book chapter and over 180 papers in refereed journals and conference proceedings.
 
Prof. Wang served or is currently serving as an editor for 8 international journals, including IEEE Transactions on Vehicular Technology (2011--) and IEEE Transactions on Wireless Communications (2007--2009). He was the Guest Editor for IEEE Journal on Selected Areas in Communications, Special Issue on Vehicular Communications and Networks and Special Issue on Spectrum and Energy Efficient Design of Wireless Communication Networks <http://www.jsac.ucsd.edu/Calls/CFP_SEED_FINAL.pdf> . He served or is serving as a TPC member, TPC Chair, and General Chair for over 70 international conferences. He received the Best Paper Awards from IEEE Globecom 2010, IEEE ICCT 2011, and ITST 2012. He is a Fellow of the IET, a Fellow of the HEA, and a member of EPSRC Peer Review College.


==> Biographies/Harald_Haas.tex <==
Professor Harald Haas (S98-A00-M03) holds the Chair of Mobile
Communications in the Institute for Digital Communications (IDCOM) at
the University of Edinburgh, and he currently is the CTO of a university
spin-out company pureVLC Ltd. His main research interests are in
interference coordination in wireless networks, spatial modulation and
optical wireless communication. Prof. Haas holds 23 patents. He has
published more than 60 journal papers including a Science Article
and more than 160 peer-reviewed conference papers. Nine of his papers
are invited papers. Prof. Haas has co-authored a book entitled ”Next
Generation Mobile Access Technologies: Implementing TDD” with Cambridge
University Press. Since 2007 Prof. Haas has been a Regular High Level
Visiting Scientist supported by the Chinese 111-program at Beijing
University of Posts and Telecommunications (BUPT). He was an invited
speaker at the TED Global conference 2011, and his work on optical
wireless communication was listed among the "50 best inventions in 2011"
in Time Magazine. He recently has been awarded a prestigious Fellowship
of the Engineering and Physical Sciences Research Council (EPSRC) in the UK.


==> Biographies/Marco_Di_Renzo.tex <==
Marco Di Renzo (S'05--AM'07--M'09) was born in L'Aquila, Italy, in 1978. He received the Laurea (cum laude) and the Ph.D. degrees in Electrical and Information Engineering from the Department of Electrical and Information Engineering, University of L'Aquila, Italy, in April 2003 and in January 2007, respectively.

From August 2002 to January 2008, he was with the Center of Excellence for Research DEWS, University of L'Aquila, Italy.
From February 2008 to April 2009, he was a Research Associate with the Telecommunications Technological Center of Catalonia (CTTC), Barcelona, Spain.
From May 2009 to December 2009, he was an EPSRC Research Fellow with the Institute for Digital Communications (IDCOM), The University of Edinburgh, Edinburgh, United Kingdom (UK).

Since January 2010, he has been a Tenured Researcher (``Charg\'e de Recherche Titulaire'') with the French National Center for Scientific Research (CNRS), as well as a faculty member of the Laboratory of Signals and Systems (L2S), a joint research laboratory of the CNRS, the \'Ecole Sup\'erieure d'\'Electricit\'e (SUP\'ELEC), and the University of Paris--Sud XI, Paris, France. His main research interests are in the area of wireless communications theory. He is a Principal Investigator of three European--funded research projects (Marie Curie ITN--GREENET, Marie Curie IAPP--WSN4QoL, and Marie Curie ITN--CROSSFIRE).

Dr. Di Renzo is the recipient of the special mention for the outstanding five--year (1997--2003) academic career, University of L'Aquila, Italy; the THALES Communications fellowship for doctoral studies (2003--2006), University of L'Aquila, Italy; the Best Spin--Off Company Award (2004), Abruzzo Region, Italy; the Torres Quevedo award for research on ultra wide band systems and cooperative localization for wireless networks (2008--2009), Ministry of Science and Innovation, Spain; the ``D\'erogation pour l'Encadrement de Th\`ese'' (2010), University of Paris--Sud XI, France; the 2012 IEEE CAMAD Best Paper Award from the IEEE Communications Society; and the 2012 Exemplary Reviewer Award from the IEEE WIRELESS COMMUNICATIONS LETTERS of the IEEE Communications Society. He currently serves as an Editor of the IEEE COMMUNICATIONS LETTERS.


==> Biographies/Mark_Beach.tex <==
Professor Mark Beach is a Professor in Radio Systems Engineering at the University of Bristol (UK). He is recognised for his research in the field of wireless communications, with specialisation in the field of multi-antenna technology for enhanced efficiency and robust wireless delivery as well as RF enabling technologies for spectrum and energy efficient connectivity He has held the post of Head of Electrical and Electronic Engineering at Bristol and now is the UK representative on EU COST IC1004 and a member of the EPSRC Strategic Advisory Team (SAT) for ICT.


==> Biographies/Nikola_Serafimovski.tex <==
Nikola Serafimovski received his B.Sc. in Electrical Engineering and Computer Science in 2007 and his M.Sc. in Communications, Systems and Electronics in 2009 from Jacobs University Bremen. He has recently completed his Ph.D. degree at the Institute for Digital Communications at the University of Edinburgh, where the focus of his research was on multiple-input multiple-output systems and the practical implementation of Spatial Modulation. He is currently working as a Communication Systems Engineer for pureVLC Ltd.


==> Biographies/Peter_Grant.tex <==
Peter M. Grant(M-77-SM-83-F-96) Peter M. Grant was born in St. Andrews, Scotland. He received the B.Sc. degree in electronic
engineering from the Heriot-Watt University, Edinburgh, Scotland, in 1966, the Ph.D. degree from the University of Edinburgh in 1975 and honorary DEng's from the Heriot-Watt in 2006 and from Napier University in 2007.

He worked in radio communications for the Plessey Company, before he was appointed to a research fellowship at the University of Edinburgh. He was subsequently promoted through to a full professor of Electronic Signal Processing and on to Departmental chair. He served from 2002-2008 as head of the School of Engineering and Electronics at Edinburgh.

During academic year 1977-78, he was a visiting professor at the Ginzton Laboratory, Stanford
University, and in 1985-86 he was a visiting staff member at the MIT Lincoln Laboratory. He was awarded the 82nd (2004) Faraday Medal by the Institution of Electrical Engineers (IEE) for his work on CDMA receiver designs and adaptive filters. In 1974 and again in 1977 he was awarded the Bulgin premium from the then Institution of Electronic and Radio Engineers and in 1982 their Lord Mountbatten premium. In 1994 he was awarded both the IEE Marconi and Langham Thompson premia.

Professor Grant was president of EURASIP in 2000-2002, he was chairman of EUSIPCO-94 and
technical programme chairman for ICASSP-89. In 1998 he was appointed by the IEEE Signal Processing Society as a distinguished lecturer on DSP for Mobile Communications. He served from 1980-1996 as an honorary editor of IEE Proceedings title "Vision Image and Signal Processing". He was a member in 1992 and 1996 and was chair of the 2001 Universities Funding Council research assessment panel for the UK Electrical Engineering Departments. He served as a director of the Mobile VCE from 2007-9.

Professor Grant was in 2007 appointed to be the 8th Regius Professor of Engineering at The University of Edinburgh.  In 2009 he was made an officer of the order of the British Empire (OBE) in the Queen's birthday honours list. He holds fellowships of the IEEE, IET, Royal Academy of Engineering and the Royal Society of Edinburgh.


==> Biographies/Raed_Mesleh.tex <==
Raed Mesleh (S'00-M'08-SM'13) Dr Mesleh holds a Ph.D. in Electrical
Engineering from Jacobs University in Bremen, Germany and several years of
post-doctoral wireless communication and optical wireless communication
research experience in Germany. In October 2010, he joined University of
Tabuk in Saudi Arabia where he is now an assistant professor and the
director of research excellence unit. His main research interests are in
spatial modulation, MIMO cooperative wireless communication techniques and
optical wireless communication. Dr Mesleh publications received more than
800 citations since 2007. He has published more than 50 publications in
top-tier journals and conferences, and he holds 7 granted patents. He also
serves as on the TPC for academic conferences and is a regular reviewer for
most of IEEE/OSA Communication Society's journals and IEEE/OSA Photonics
Society's journals.

